Reaching the End of Unbiasedness: Uncovering Implicit Limitations of Click-Based Learning to Rank

Click-based learning to rank (LTR) tackles the mismatch between click frequencies on items and their actual relevance. The approach of previous work has been to assume a model of click behavior and to subsequently introduce a method for unbiasedly estimating preferences under that assumed model. The success of this approach is evident in that unbiased methods have been found for an increasing number of behavior models and types of bias. This work aims to uncover the implicit limitations of the high-level prevalent approach in the counterfactual LTR field. Thus, in contrast with limitations that follow from explicit assumptions, our aim is to recognize limitations that the field is currently unaware of. We do this by inverting the existing approach: we start by capturing existing methods in generic terms, and subsequently, from these generic descriptions we derive the click behavior for which these methods can be unbiased. Our inverted approach reveals that there are indeed implicit limitations to the counterfactual LTR approach: we find counterfactual estimation can only produce unbiased methods for click behavior based on affine transformations. In addition, we also recognize previously undiscussed limitations of click-modelling and pairwise approaches to click-based LTR. Our findings reveal that it is impossible for existing approaches to provide unbiasedness guarantees for all plausible click behavior models.

==> 04-counterfactual.tex <==

\section{Methodology}
\label{sec:method}

Section~\ref{sec:background} described the prevalent approaches in the unbiased \ac{LTR} field and noted that the limitations of the high-level approach are currently unclear.
In this work, we will investigate whether there are implicit assumptions in the two main families of debiasing approaches.
In particular, we want to find out whether they impose limits on which circumstances estimation methods can or cannot be unbiased or consistent. 
This section will explain our methodology to investigating such implicit limitations, we will start by defining the two theoretical properties that we are interested in.

We begin by formally defining unbiasedness:
\begin{definition}
\label{def:unbiasedness}
\emph{Unbiasedness.}
A click-based relevance estimation method is \emph{unbiased}, if the expected values of all the resulting relevance estimates are equal to the true relevances:
\begin{equation}
\forall (d, q),\;
\mathbb{E}\big[ \hat{R}_{d|q} \big] = R_{d|q}.
\end{equation}
\end{definition}
Our definition is slightly different than the standard definition in the previous literature:
where existing work has focussed on the estimated performance of a ranking system (Eq.~\ref{eq:existingunbiassystem})~\citep{joachims2017unbiased, oosterhuis2020thesis, agarwal2019counterfactual}, we focus on bias of the individual relevance estimates.
We motivate this difference with three arguments:
\begin {enumerate*} [label=(\roman*)]
\item Our definition based on individual relevance estimates practically guarantees an unbiased performance estimate (c.f.\ Eq.~\ref{eq:rankingquality});
\item To the best of our knowledge, there is no existing work that provides an unbiased performance estimate without also providing unbiased relevance estimates~\citep{wang2016learning, joachims2017unbiased, oosterhuis2020thesis, agarwal2019counterfactual, oosterhuis2020topkrankings, vardasbi2020trust, oosterhuis2021onlinecounterltr, ai2018unbiased, hu2019unbiased, wu2021unbiased, vardasbi2020cascade}.
In other words, all existing unbiased \ac{LTR} methods are also unbiased under our definition.
\item Our definition is simpler and easier to work with.
\end{enumerate*}
To summarize, we define unbiasedness based on individual relevance estimates because it is easier to work with and is interchangeable with the unbiased definition based on system performance in previous work.

While unbiasedness has been the main focus of most click-based \ac{LTR} work, it is not the only property that is important to the field.
As Section~\ref{sec:shortcomings} noted, in practice counterfactual estimation methods are often deployed in a biased manner.
In particular, propensity clipping introduces some bias but reduces variance greatly and is widely applied in counterfactual \ac{LTR}~\citep{joachims2017unbiased, agarwal2019addressing, oosterhuis2021onlinecounterltr, vardasbi2020trust, oosterhuis2020topkrankings}.
Similarly, it is conceptually hard to apply the unbiasedness property to click modelling methods~\citep{vardasbi2021mixture}.
For these reasons, we will also consider \emph{consistency}~\citep{oosterhuis2020taking} with the following formal definition:
\begin{definition}
\label{def:consistency}
\emph{Consistency.}
A click-based relevance estimation method is \emph{consistent}, if the values of all the resulting relevance estimates are equal to the true relevances in the limit of an infinite number of interactions:
\begin{equation}
\lim_{|\mathcal{D}_q| \to \infty} \hat{R}_{d|q} = R_{d|q}.
\end{equation}
\end{definition}
Consistency is a desirable property since it guarantees accurate convergence as interaction data continues to increase.
Furthermore, variance is generally negligible when the number of interaction is extremely large~\citep{joachims2017unbiased}, therefore unlike unbiasedness, there is often not a trade-off between variance and consistency.

Our goal is thus to identify under which conditions the unbiased \ac{LTR} approach can provide methods that are unbiased and consistent according to our definitions.
Our method to identifying these conditions inverts the prevalent approach that starts with behavior assumptions and derives an unbiased method.
In contrast, we first describe the two main families: counterfactual estimation and click modelling, in the most generic terms.
Subsequently, we derive click behavior conditions from these generic methods, thereby revealing the assumptions that are implicitly present in the existing approach.
The following two sections will do this for counterfactual estimation and click modelling, in addition, Section~\ref{sec:othermethods} will discuss other methods that fall outside the former two categories.

\section{The Limitations of Click-Based Counterfactual Estimators}
\label{sec:limitcount}

As discussed in Section~\ref{sec:existingcounterfactual}, counterfactual estimation represents the largest branch of the unbiased \ac{LTR} field~\citep{wang2016learning, joachims2017unbiased, oosterhuis2020thesis}.
The underlying assumption of these methods is that click probabilities are decomposable into relevance and display factors, e.g.\ the estimator in Eq.~\ref{eq:existingcfest} assumes click probabilities are determined by relevance and display-position according to Eq.~\ref{eq:affineclickmodel}~\citep{vardasbi2020trust}.
Click-based counterfactual estimators aim to convert a click signal into an unbiased relevance signal by correcting for the display factors.
In order to investigate the entire family of click-based counterfactual estimators, we first define a display context $x(d)$ in the most generic and broad terms:
\begin{definition}
\label{def:displaycontext}
\emph{Display Context.}
The display context $x_i(d)$ contains all information about how item $d$ is displayed that could affect the click probability of $d$ at interaction $i$.
It does not contain any information about the relevance $d$: $R_{d|q}$.
In other words,
one should be able to determine $x_i(d)$ without any knowledge of $R_{d|q}$.
\end{definition}
For example, for the estimator in Eq.~\ref{eq:existingcfest} the display context is the display position: $x_i(d) = k_i(d)$~\citep{agarwal2019addressing}. 
Many alternatives are possible, e.g.\ $x_i(d)$ can also represent a probability distribution over positions as in the policy-aware estimator ~\citep{oosterhuis2020topkrankings, oosterhuis2021onlinecounterltr}.
With this broad definition of the display context, we propose a generic description of a click-based counterfactual estimator:
\begin{definition}
\label{def:counterfactualestimate}
\emph{Counterfactual Relevance Estimate.}
A click-based counterfactual relevance estimate is an average over independently sampled interactions where each click or non-click is transformed by a function $f$ such that:
\begin{equation}
\hat{R}_{d|q} = \frac{1}{N_q}\sum_{i \in \mathcal{D}_q} f(c_i(d), x_{i}(d)).
\label{eq:counterfactualestimate}
\end{equation}
Accordingly, $f$ only has two relevant values per context $x(d)$ for the counterfactual estimate:
$f(1, x(d))$ when a click takes place on $d$ and $f(0, x(d))$ when no click takes place.
\end{definition}
To the best of our knowledge, Definition~\ref{def:counterfactualestimate} covers all existing click-based counterfactual estimators~\citep{wang2016learning, joachims2017unbiased, oosterhuis2020topkrankings, vardasbi2020trust, oosterhuis2020thesis, agarwal2019counterfactual, agarwal2019addressing, oosterhuis2021onlinecounterltr, ai2018unbiased, wu2021unbiased, vardasbi2020cascade} with the exception of three counterfactual pairwise estimators~\citep{wang2021non, hu2019unbiased, saito2020unbiased} that will be discussed in Section~\ref{sec:othermethods}.
For example, we see that the estimator in Eq.~\ref{eq:existingcfest} is a specific instance where $f$ is chosen so that $f(1,x_i(d)) = \frac{1- \beta_{k_i(d)}}{\alpha_{k_i(d)}}$ and $f(0,x_i(d)) = \frac{- \beta_{k_i(d)}}{\alpha_{k_i(d)}}$.
The aim of our definition is to cover all existing estimators and as many future estimators as possible.
Accordingly, - to the best of our knowledge - different choices of $f$ can cover almost all existing counterfactual estimators, and moreover, they can also cover many more possible estimators that have yet to be introduced to the field.

With these definitions, we can now start to derive the conditions for which a click-based counterfactual estimator is unbiased or consistent.
First, we note that the expected value of a relevance estimate $\hat{R}_{d|q}$ is simply the expected value of $f$ conditioned on $q$:
\begin{lemma}
\label{lemma:cfest:expected}
In expectation a counterfactual relevance estimate is:
\begin{equation}
\mathbb{E}_{c,x}\mleft[ \hat{R}_{d|q} \mright] 
= \mathbb{E}_{c,x}\mleft[ f(c(d), x(d)) \mid q \mright].
\end{equation}
\end{lemma}
\begin{proof} Using Definition~\ref{def:counterfactualestimate}:
\begin{align}
&\mathbb{E}_{c,x}\mleft[ \hat{R}_{d|q} \mright]
= \mathbb{E}_{c,x}\bigg[ \frac{1}{N_q}\sum_{i \in \mathcal{D}_q} f(c_i(d), x_{i}(d)) \bigg]
\\
&= \mathbb{E}_{c,x}\mleft[ f(c_i(d), x_{i}(d)) \mid i \in D_q \mright]
= \mathbb{E}_{c,x}\mleft[ f(c(d), x(d)) \mid q \mright]. \qedhere
\end{align}
\end{proof}
With this Lemma, we can prove that an unbiased estimator is always consistent and vice-versa:
\begin{theorem}
\label{theorem:cfbiasandcons}
A counterfactual estimator is consistent if and only if it is unbiased:
\begin{equation}
\mathbb{E}_{c,x}\mleft[ \hat{R}_{d|q} \mright] = R_{d|q} \longleftrightarrow \lim_{|\mathcal{D}_q| \to \infty} \hat{R}_{d|q} = R_{d|q}.
\end{equation}
\end{theorem}
\begin{proof}
With the use of Definition~\ref{def:counterfactualestimate} and Lemma~\ref{lemma:cfest:expected}:
\begin{equation}
\lim_{|\mathcal{D}_q| \to \infty} \hat{R}_{d|q}
= \mathbb{E}_{c,x}\mleft[f(c_i(d), x_{i}(d)) \mid q \mright]
= \mathbb{E}_{c,x}\mleft[ \hat{R}_{d|q} \mright].
\qedhere
\end{equation}
\end{proof}
Therefore, it appears that the focus of previous work to prove unbiasedness was not incorrectly placed, since implicitly this has also proved consistency.
Nevertheless, we think it is important that we have a theoretical motivation for this focus now.
Finally, we can derive the following conditions for the unbiasedness - and therefore also the consistency - of click-based counterfactual estimators:
\begin{theorem}
\label{theorem:counterestimateunbiased}
\label{theorem:cf}
A counterfactual estimator can only be unbiased if click probabilities follow an affine transformation of relevance s.t:
\begin{equation}
\label{eq:counter:clickprobaffine}
R_{d|q} =
\mathbb{E}_{x}\mleft[ 
\frac{P(C =1 \mid d, x, q) - \beta_{x(d)}}{\alpha_{x(d)}}
\mid q\mright].
\end{equation}
\end{theorem}
\begin{proof}
From Lemma~\ref{lemma:cfest:expected} it follows that the unbiasedness criteria for a counterfactual relevance estimate can be reformulated as:
\begin{equation}
\mathbb{E}_{c,x}\mleft[ \hat{R}_{d|q} \mright] = R_{d|q} \longleftrightarrow
\mathbb{E}_{c,x}\mleft[ f(c(d), x({d})) \mid q \mright] = R_{d|q}.
\label{eq:countercrit1}
\end{equation}
The expected value can be rewritten to:
\begin{align}
&\mathbb{E}_{c,x}\mleft[ f(c(d), x({d})) \mid q \mright]
\label{eq:expectrewrit}\\&
=
\mathbb{E}_{x}[ 
P(C =1 \mid d, x, q)f(1, x({d}))
\nonumber\\
&\hspace{3.3cm} + (1 - P(C =1 \mid d, x, q))f(0, x({d}))
\mid q]
\nonumber\\&
=
\mathbb{E}_{x}\mleft[ 
P(C =1 \mid d, x, q)(f(1, x({d})) - f(0, x({d}))) + f(0, x({d}))
\mid q\mright].
\nonumber
\end{align}
Combining Eq.~\ref{eq:countercrit1} and~\ref{eq:expectrewrit} reveals that the unbiasedness criteria also has implications on the click probability: 
\begin{align}
\mathbb{E}_{c,x}\big[ \hat{R}_{d|q} \big] = R_{d|q} \longleftrightarrow
\mathbb{E}_{x}&\big[
P(C =1 \mid d, x, q)(f(1, x({d}))
\label{eq:theorem55lasteq}
\\&
- f(0, x({d}))) + f(0, x({d}))
\mid q\big]
=
R_{d|q}.
\nonumber
\end{align}
To prove Theorem~\ref{theorem:counterestimateunbiased}, we derive the following $\alpha_{x(d)}$ and $\beta_{x(d)}$  from Eq.~\ref{eq:theorem55lasteq} which
show that click probability is an affine transformation of the form stated in Eq.~\ref{eq:counter:clickprobaffine}:
\begin{align}
\alpha_{x(d)} &= (f(1, x({d})) - f(0, x({d})))^{-1},
\label{eq:alphabetavalueproof}
\\
\beta_{x(d)} &= -f(0, x({d}))(f(1, x({d})) - f(0, x({d})))^{-1}.\qedhere
\end{align}
\end{proof}
Theorem~\ref{theorem:cf} can be difficult to interpret since the expectation over the display context in Eq.~\ref{eq:counter:clickprobaffine} depends on the choice of logging policy.
Nonetheless, Theorem~\ref{theorem:cf} clearly shows that - in spite of being broad and generic - Definition~\ref{def:counterfactualestimate} implicitly limits the click models counterfactual relevance estimation can be unbiased or consistent for.
It appears that this is a result of the estimate being a mean over individually transformed clicks (Eq.~\ref{eq:counterfactualestimate}) which makes its expected value a linear interpolation between the possible $f(0, x(d))$ and $f(1, x(d))$ values.
Consequently, an counterfactual estimator following Definition~\ref{def:counterfactualestimate} can only be unbiased or consistent if clicks follow a transformation that can be corrected by such an interpolation, Theorem~\ref{theorem:cf} proves that such a transformation has to match the affine form of Eq.~\ref{eq:counter:clickprobaffine}.

To better understand what Theorem~\ref{theorem:cf} entails, we consider what it would mean for a deterministic logging policy:
\begin{corollary}
\label{corollary:cfnorandom}
If an item is displayed without randomization then a counterfactual estimator can only be unbiased if the item's click probability is an affine transformation of relevance in the form:
\begin{equation}
P(x(d) \mid q) = 1 \rightarrow 
P(C =1 \mid d, x, q) = \alpha_{x(d)} R_{d|q} + \beta_{x(d)}.
\label{eq:counter:clickprobaffinenorandom}
\end{equation}
\end{corollary}
\begin{proof}
This follows directly from Theorem~\ref{theorem:cf}.
\end{proof}
Furthermore, often practitioners have no control over the exact logging policy that gathers data.
In such a scenario, unbiasedness guarantees cannot rely on a specific choice of logging policy as the deployment of that policy may not be possible:
\begin{corollary}
\label{corollary:cfstrong}
Without control over the logging policy, unbiasedness guarantees for a counterfactual estimator are only possible if click probabilities are affine transformations of relevance in the form:
\begin{equation}
 \forall (d, x, q), \;
P(C =1 \mid d, x, q) = \alpha_{x(d)} R_{d|q} + \beta_{x(d)}.
\label{eq:counter:clickprobaffinestrong}
\end{equation}
\end{corollary}
\begin{proof}
We cannot rule out the possibility that for each possible display context an item exists which the logging policy will only display in that context, thus, Cor.~\ref{corollary:cfstrong} follows from Cor.~\ref{corollary:cfnorandom}.
\end{proof}
While the individual steps of our theoretical derivation are very straightforward, the result is quite significant:
we have proven that the form of click-based counterfactual estimators entail implicit assumptions about the click behavior they are able to unbias.
In other words, because click-based counterfactual estimators transform individual click or non-click signals and then average the result, they can only correct for click probabilities that are affine transformations of relevances.
Conversely, this proves that no unbiased counterfactual relevance estimator (Def.~\ref{def:counterfactualestimate}) can exist for click behavior that does not match the affine transformation of Eq.~\ref{eq:counter:clickprobaffine}.

Furthermore, there is a less obvious implicit requirement that $\alpha_{x(d)}$ and $\beta_{x(d)}$ should only depend on the display context and not on the item relevance:
\begin{corollary}
\label{corollary:cf}
If two items are always displayed in the same single display context, their $\alpha_{x(d)}$ and $\beta_{x(d)}$ values should be equal:
\begin{equation}
\begin{split}
&\big(\exists x', \, P(x(d) = x' \mid q ) = 1 \land P(x(d') = x' \mid q ) = 1 \big) 
\\&\hspace{1.2cm} \longrightarrow
P\big(\alpha_{x(d)} = \alpha_{x(d')} \land \beta_{x(d)} = \beta_{x(d')} \mid q \big) = 1.
\end{split}
\end{equation}
\end{corollary}
\begin{proof} 
According to Definition~\ref{def:displaycontext}, $x(d)$ is not determined by the relevance of $d$.
Therefore, two items with the same display context $x(d)$ should also have the same values from $f$:
\begin{equation}
\begin{split}
&\big(x(d) = x(d')\big) \leftrightarrow \big(f(0, x(d)) = f(0, x(d'))
\\
&\hspace{3.1cm} \land f(1, x(d)) = f(1, x(d'))\big).
\end{split}
\end{equation}
Cor.~\ref{corollary:cfnorandom} and
Eq.~\ref{eq:alphabetavalueproof} show $\alpha_{x(d)}$ and $\beta_{x(d)}$ must then be equal.
\end{proof}
This requirement becomes more obvious when one considers the implications of its negation: a setting where the value of $\alpha_{x(d)}$ and $\beta_{x(d)}$ are determined by $R_{d|q}$.
In such a setting the value of $f(0, x(d))$ and $f(1, x(d))$ are also determined by $R_{d|q}$, and therefore, one should first know the relevance of an item before being able to unbiasedly estimate it.
In other words, in such a setting one can only unbiasedly estimate relevances if one already knows those relevances and thus has no need for estimation.
Importantly, we are not arguing that such settings do not exist but merely that unbiased counterfactual estimation is infeasible in such cases.

In addition to the requirement stated in Theorem~\ref{theorem:cf} and Corollaries~\ref{corollary:cfnorandom}, \ref{corollary:cfstrong} and~\ref{corollary:cf}, there could be more requirements that have yet to be proven.
In particular, our analysis has not considered under what conditions the values of $f$ or $\alpha$ and $\beta$ can be determined.
Previous work on position-bias estimation~\citep{wang2018position, agarwal2019estimating, craswell2008experimental, chuklin2015click} shows that bias estimation is far from a trivial task.
Therefore, it seems reasonable that it is also necessary that the bias parameters $\alpha$ and $\beta$ can be accurately inferred  for unbiased counterfactual estimation.
However, we currently lack a theoretical approach to prove broad conditions about bias estimation in general (Section~\ref{sec:biasestimationcm} will discuss bias estimation with click modelling).

To summarize our theoretical findings on counterfactual estimation for click-based \ac{LTR}:
We have provided a generic definition of click-based counterfactual estimators that captures almost all methods in the field~\citep{wang2016learning, joachims2017unbiased, oosterhuis2020topkrankings, vardasbi2020trust, oosterhuis2020thesis, agarwal2019counterfactual, agarwal2019addressing, oosterhuis2021onlinecounterltr, ai2018unbiased, wu2021unbiased, vardasbi2020cascade}.
From this definition, we have shown that estimators of this form can only provide unbiased and consistent estimates when click probabilities are affine transformations of relevances.
We have thus identified a significant limitation of the high-level approach for click-based counterfactual estimation: it can never find unbiased or consistent methods for non-affine click behavior.

The remainder of this section will provide some example scenarios that illustrate this limitation and discuss some edge-cases related to our definitions.

\begin{figure}[tb]
\centering
{\renewcommand*{\arraystretch}{0.4}
\begin{tabular}{r c}
\rotatebox[origin=c]{90}{
\hspace{-1cm}
\small
Click Probability
\hspace{-4cm}
}
& \includegraphics[scale=0.475]{figures/cf_example.pdf}\\
\multicolumn{2}{c}{\hspace{0.5cm}
\small
Item Relevance
}
\end{tabular}
}
\caption{
The relation between click probability and relevance in the Plackett-Luce and cascading scenarios of Section~\ref{sec:cfscenario}.
}
\vspace{-\baselineskip}
\label{fig:cfexample}
\end{figure}

\subsection{Example Scenarios}
\label{sec:cfscenario}

To better understand what the implicit limitations of counterfactual estimation regarding affine click-behavior entail,
we will briefly discuss two models of click behavior that illustrate scenarios where unbiased estimation is possible and impossible.

To start, we will consider a model of behavior where a user first considers all items in a ranking and then chooses according to a Plackett-Luce decision model:
\begin{equation}
P_\text{plackett-luce}(c(d) = 1 \mid y, q) = \frac{\mathds{1}[d \in y] \cdot R_{d|q}}{\sum_{d' \in y} R_{d'|q}}.
\end{equation}
Thus the probability of a user choosing an item in a ranking is equal to its relevance divided by the sum of the relevances of all items in the ranking.
This Plackett-Luce click model is based on well-established decision models from the economic field~\citep{plackett1975analysis, luce2012individual}.
To keep our example simple, we have not added any form of position-bias or trust-bias in the model, although such extensions are certainly possible.

At first glance the Plackett-Luce click model may incorrectly seem to fall within the limitations of counterfactual estimation with the following parameters:
$\alpha_{x(d)} = \mathds{1}[d \in y]/\sum_{d' \in y}  R_{d'|q}$ and $\beta_{x(d)} = 0$ (cf.\  Eq.~\ref{eq:counter:clickprobaffinenorandom}).
However, the denominator of this $\alpha_{x(d)}$ is directly determined by the relevances of \emph{all} items in the ranking, thus also by the item for which relevance is estimated itself.
It therefore does not match the definition of an affine click-model.
This can be clearly seen when plotting how the click probability changes with an item's relevance; Figure~\ref{fig:cfexample} displays this for a scenario where the other relevances that sum up to $0.01$: $\sum_{d' \in y / d} R_{d'|q} = 0.01$.
Clearly, there is not an affine transformation from relevance to click probabilities, and consequently, it is impossible for a click-based counterfactual estimator according to Definition~\ref{def:counterfactualestimate} to provide an unbiased or consistent estimate in this scenario.


This does not mean that unbiased counterfactual estimation is impossible for all click models where click probabilities depend on the relevances of other items.
For example, let us consider a classic cascading click model where a user considers one item at a time until one is clicked~\citep{chuklin2015click, craswell2008experimental}.
The click probability is thus:
\begin{equation}
\begin{split}
&P_\text{casc}(c(d) = 1 \,|\, d, y, q) 
\\%[-1.2ex]
&\hspace{0.5cm} = P_\text{casc}(\forall d' \in y, \, k(d') < k(d) \rightarrow c(d') = 0 \,|\, y, q) \cdot R_{d|q}.
\end{split}
\end{equation}
Therefore. this scenario does provide an affine transformation with $\alpha_{x(d)} = P_\text{casc}(\forall d' \in y, \, k(d') < k(d) \rightarrow c(d') = 0 |\, y, q)$ -- the probability that no earlier item was clicked -- and $\beta_{x(d)} = 0$ (cf.\  Eq.~\ref{eq:counter:clickprobaffinenorandom}).
Figure~\ref{fig:cfexample} also shows how the click probability changes with relevance in a scenario where $\alpha_{x(d)} =0.7$, which clearly reveals an affine transformation.
The crucial difference in this scenario is that the value of $\alpha_{x(d)}$ only depends on other items and not on $d$ itself.

These examples illustrate an intuitive way to think of Theorem~\ref{theorem:cf}:
unbiasedness and consistency guarantees for counterfactual estimation are only possible if there is a linear relation between click probability and item relevance.


\subsection{Adaptive Normalization and Clipping}

While our definition of counterfactual relevance estimates (Definition~\ref{def:counterfactualestimate}) covers almost all click-based counterfactual estimators, it does not fit perfectly with adaptive self-normalization~\citep{swaminathan2015self} and clipping strategies that change with $|\mathcal{D}_q|$~\citep{oosterhuis2021onlinecounterltr, oosterhuis2020topkrankings}.
For instance, a popular clipping strategy is one where $\lim_{|\mathcal{D}_q| \to \infty} \tau = 0$, e.g.\ with $\tau \propto 1/\sqrt{|\mathcal{D}_q|}$~\citep{oosterhuis2021onlinecounterltr, oosterhuis2020topkrankings}.
To incorporate these exceptions one could use the function: 
$f(c_i(d),\allowbreak x_{i}(d),\allowbreak |\mathcal{D}_q|)$
in Definition~\ref{def:counterfactualestimate}.
This change would mean unbiasedness now has to be proven for all possible $|\mathcal{D}_q|$ values, and consistency only requires unbiasedness in the limit, i.e.\ $\lim_{|\mathcal{D}_q| \to \infty} \mathbb{E}[\hat{R}_{d|q}] = R_{d|q}$.
In spite of these differences, Theorem~\ref{theorem:cf} would only need minor changes and the main point would still hold: unbiasedness and consistency are only possible under affine click behavior.
We argue that the simplicity of our theoretical analysis with Definition~\ref{def:counterfactualestimate} and the lack of significant implications of including adaptive strategies, justify our choice of excluding them.
